One Energy Game for the Spectrum between Branching Bisimilarity and Weak Trace Semantics

We provide the first generalized game characterization of van Glabbeek's linear-time--branching-time spectrum with silent steps. Thereby, one multi-dimensional energy game can be used to characterize and decide a wide array of weak behavioral equivalences between stability-respecting branching bisimilarity and weak trace equivalence in one go. To establish correctness, we relate attacker-winning energy budgets and distinguishing sublanguages of Hennessy--Milner logic that we characterize by eight dimensions of formula expressiveness.

==> eptcsdata.tex <==
\providecommand{\firstpage}{71}
\providecommand{\publicationstatus}{G. Caltais and C. Di Giusto (Eds.): EXPRESS/SOS 2024\\
EPTCS 412, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.412.6}{10.4204/EPTCS.412.6}}
\pdfoutput=1


==> silent-step-spectroscopy_express-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\prAtEndRestateiii*

\prAtEndRestateiv*

\prAtEndRestatev*

